Efficient Algorithms for Finite Horizon and Streaming Restless Multi-Armed Bandit Problems

We propose Streaming Bandits, a Restless Multi Armed Bandit (RMAB) framework in which heterogeneous arms may arrive and leave the system after staying on for a finite lifetime. Streaming Bandits naturally capture the health intervention planning problem, where health workers must manage the health outcomes of a patient cohort while new patients join and existing patients leave the cohort each day. Our contributions are as follows: (1) We derive conditions under which our problem satisfies indexability, a precondition that guarantees the existence and asymptotic optimality of the Whittle Index solution for RMABs. We establish the conditions using a polytime reduction of the Streaming Bandit setup to regular RMABs. (2) We further prove a phenomenon that we call index decay, whereby the Whittle index values are low for short residual lifetimes driving the intuition underpinning our algorithm. (3) We propose a novel and efficient algorithm to compute the index-based solution for Streaming Bandits. Unlike previous methods, our algorithm does not rely on solving the costly finite horizon problem on each arm of the RMAB, thereby lowering the computational complexity compared to existing methods. (4) Finally, we evaluate our approach via simulations run on realworld data sets from a tuberculosis patient monitoring task and an intervention planning task for improving maternal healthcare, in addition to other synthetic domains. Across the board, our algorithm achieves a 2-orders-of-magnitude speed-up over existing methods while maintaining the same solution quality.

==> UAI/old_text.tex <==
%Rough outline to expand: We start with talking about the health monitoring and intervention planning problem as our motivation. We say that Restless bandits have been used popularly to address such kind of limited resource problems in the past [refs] especially the HMIP [cite Collapsing Bandits etc]. However these models (CoB) are limited to large horizon settings and deteriorate for smaller horizons. Further exacerbated when everyone doesn't arrive at the same time but rather arrives asynchronously—which is the case in real world..patients etc. But exact algorithms like Qian et al. cant address this problem because very slow. SO we solve this problem and present (two) new algorithms that are faster. We achieve a [insert here] times speedup without sacrificing on performance 


%<This section may go to RELATED WORK>Recent work has paid has casted the health monitoring and intervention planning problems as a restless bandit problem \cite{mate2020collapsing, mate2021riskAware}.  In HMIP, a heath worker monitors the health of a cohort of patients and intervenes on patients in the bad state to try and push them to the good state. Because of severe resource constraints, the health worker can't intervene on everybody and thus faces this sequential planning problem of deciding which patients to intervene on. 

%<This section may go to RELATED WORK>A fairly general approach, proposed by \cite{qian2016restless}, adopts the Whittle Index policy for health intervention planning. More recent approaches, proposed by~\cite{mate2020collapsing,mate2021riskAware} exploit the structure of the HMIP and are dramatically faster but these rely on the planning horizon being very large/infinite. These fast algorithms suffer a severe deterioration in performance when applied to finite horizon settings.


%Existing RMAB algorithms for health intervention planning adopt the Whittle Index approach and are fairly general, but consequently very slow \cite{qian2016restless}. More recent approaches exploit the structure of the HMIP and are dramatically faster but these rely on the planning horizon being very large/infinite. These fast algorithms suffer a severe deterioration in performance when applied to finite horizon settings. The issue is further exacerbated when the planning horizon doesn't begin at the same time for different arms — which is characteristic of the real world, in which patients enroll into health programs or leave upon completion on a rolling basis. The more general approaches can tackle both these issues but are just too slow to run. 






















% \subsection{Synchronous Arms, Randomly Sleeping}
%  We have an RMAB with $N$ arms, all of them starting at $t=0$ with some horizon $L$ and a budget to pull $k$ of these arms each day. However, upon pulling an arm, we may discover it to be sleeping. Let $p_{sleep}^i$ be the probability that the $i^{th}$ arm is sleeping on any given day. 
% \subsection{Asynchronous Arms, Deterministic sleeping at end-of-lifetime}
% At each timestep, we have $X_t$ new arms joining the system. Each arm $i$ remains available in the system for $L_i$ time steps and then goes to sleep for good. This process goes on for a total of $L (L \gg L_i)$ timesteps. We always have a budget of $k$ arms to pull. 


%\section{Random Sleeping}


% \begin{figure}[t!]
% \centering
% \resizebox{!}{100pt}{%
% \begin{tikzpicture}[
%     % start chain = going right,
%     -Triangle, every loop/.append style = {-Triangle},
%     start chain=main going right,
%     state/.style={circle,minimum size=8mm,draw},
%     % every node/.style=draw,
%       % minimum size=2cm,
%       % max size=5mm,
%       node distance=8mm,
%       font=\scriptsize,
%       >=stealth,
%       bend angle=28,
%       auto
%     ]
%   \node [state, on chain, fill=black, text=white] (1) {\textbf{$b_0$(1)}};
%   {[start branch=A going below]
%   \node[state, on chain, fill=black, text=white]  (A) {\textbf{$b_1$(1)}};
%   }
%   \node [state, on chain] (2) {$b_0$(2)};
%   {[start branch=A going below]
%   \node[state, on chain]  (B) {$b_1$(2)};
%   }
%     \node [state, on chain] (3) {$b_0$(3)};
%   {[start branch=A going below]
%   \node[state, on chain, fill=lightgray]  (C) {$b_1$(3)};
%   }
%   \node[state, on chain, fill=lightgray]  (4) {$b_0$(4)};
%   {[start branch=A going below]
%   \node[state, on chain]  (D) {$b_1$(4)};
%   }
%   \node[state, on chain]  (5) {...};
%   {[start branch=A going below]
%   \node[state, on chain]  (E) {...};
%   }
% %   \node[state, on chain]  (L) {$b_0$(L))};
% %   {[start branch=A going below]
% %   \node[state, on chain]  (E) {$b_1$(L)};
% %   }

%   \foreach \i in {1,...,2} {
%      \draw let \n1 = { int(\i+1) } in
%       (\i)  edge[] (\n1);
%     %   (\n1) edge[bend left] (\i);
%   }
%   \draw (3)  edge[] (4);
% %   \draw (i)  edge[] (L);
  

%   \draw (A) edge[](B);
%   \draw (B) edge[] (C);
% %   \draw (C) edge[] (D);
% %   \draw (D) edge[] (E);
  
%   \path[->,draw, thick]
%     (C) edge node[near end] {$(1-p_{sleep})(1-b_1(3))$} (1);
    
% \path[->,draw, thick, bend right=45, red]
%     (C) edge node[below] {$p_{sleep}(1-b_1(3))$} (D);    
    
%     \path[->,draw, thick, bend left=25]
%     (C) edge node[near start] {$b_1(3)$} (A);
    
%     \path[->,draw, thick, bend right=25]
%     (4) edge node[near end, above] {$(1-p_{sleep})(1-b_0(4))$} (1);
    
%     \path[->,draw, thick, bend left=45, red]
%     (4) edge node[near end, above] {$p_{sleep}(1-b_0(4))$} (5);
    
%     \path[->,draw, thick]
%     (4) edge node[near start] {$(1-p_{sleep})(b_0(4))$} (A);
 
% \end{tikzpicture}
% }
% \caption{State transition diagram when a threshold policy with thresholds $u_0=4$ and $u_1=3$ is implemented. Belief stochastically resets to one of the reset states when active.}
% \label{fig:bMDPThresholdPolicy}
% \end{figure}


% \subsection{Theoretical results?}
% \begin{equation}
%     \label{eq:discounted_value_fn_definition}
%     \begin{split}
%         V_m(b) = \max
%         \begin{cases}
%         V_{pass} & \text{passive} \\
%         V_{act}& \text{active} 
%         \end{cases}
%     \end{split}
% \end{equation}
% \begin{align}
%     \text{where:}&\\
%     &V_{pass}= m+b+\beta V_m(\tau_1(b)) \\
%     & V_{act}= b + (1-p_{sleep})\Big(\beta(bV_m(P_{1,1}^a) + \\ & (1-b)V_m(P_{0,1}^a)) \Big) + p_{sleep} \Big(\beta V_m(\tau_1(b))\Big)
% \end{align}

% \begin{theorem}\label{thm:fwd_threshold_opt}
% Consider a belief state MDP induced by arm of the RMAB which receives a subsidy of $m$ when not pulled, and may turn out to be sleeping with a probability $P_{sleep}$ when pulled. Then for such a belief state MDP, the optimal policy (as a function of $m$ and $p_{sleep}$) is a \textit{forward} threshold policy if: <some condition>  
% [The way to derive the condition and the proof seems to be following the proof process in \cite{mate2021riskAware}.]
% \end{theorem}

% \begin{theorem}\label{thm:rev_threshold_opt}
% Consider a belief state MDP induced by arm of the RMAB which receives a subsidy of $m$ when not pulled, and may turn out to be sleeping with a probability $P_{sleep}$ when pulled. Then for such a belief state MDP, the optimal policy (as a function of $m$ and $p_{sleep}$) is a \textit{reverse} threshold policy if: <some condition> 

% \end{theorem}

% \begin{theorem}\label{thm:indexability_maintext}
% If for each arm and any subsidy $m \in \mathbb{R}$, there exists an optimal policy that is a forward or reverse threshold policy, the RMAB with randomly sleeping arms is indexable under discounted and average reward criteria.
% [This theorem may possibly directly follow from the Collapsing Bandits proof \citet{mate2020collapsing}, there may be nothing new to do. Have to check.]
% \end{theorem}

